An Extensive Survey on the Internet of Drones

The Internet of Drones (IoD) recently gained momentum due to its high adaptability to a wide variety of complex scenarios. Indeed, Unmanned Aerial Vehicles (UAVs) can successfully be employed in different applications, thanks to some technological and practical advantages: high mobility, capability to extend wireless coverage areas, or ability to reach places inaccessible to humans. Moreover, the employment of drones promisingly improves the performance parameters of different network architectures. Nevertheless, the adoption of networks of drones gives rise to several issues related to the unreliability of the wireless medium, the duration of batteries, and the high mobility degree, which may cause frequent topology changes. Also security and privacy issues need to be properly investigated. With respect to other surveys on IoD-related topics, the goal of the present work is to categorize the multifaceted aspects of IoD, proposing a classification approach of the IoD environment that develops along two main directions. At a macroscopic level, it follows the structure of the Internet protocol stack, starting from the physical layer and extending to the upper layers, without neglecting cross-layer and optimization approaches. At a finer level, all the most relevant works belonging to each layer of the stack are further classified, according to the different issues peculiar of the layer, and highlighting the most relevant differences with the other surveys present in literature. To provide a deeper insight in the theme, the present work embraces many facets of the IoD, including privacy and security considerations as well as the potential economic impact of the IoD. Finally, a discussion on the main research challenges and possible future directions is carried out, focusing on the open issues and the most promising technologies that deserve to be further developed in the IoD field.

==> src/old/9-future.tex <==
\section{Research Perspectives}\label{sec:research}
In this section, the main research challenges and possible future directions in the \ac{IoD} field are highlighted.

First of all, it is worth remarking that on top of the layered structure proposed so far, many considerations can be done on the possible intersections between two or more of the reported layers.
Unmanned vehicles could represent a technological aid in the development of cellular networks as they are conceived today. Mobile base stations could sensibly enhance and improve both network capacity and coverage, especially in highly dense urban scenarios and/or crowded areas, as happens during concerts and/or important sport events in stadiums. In these use-cases, in fact, the cellular infrastructure could be offloaded with minimal preliminary effort spent for network planning activities. These considerations suggest to direct further research efforts towards the integration and inter-operation of different network architectures.

Other efforts could be spent in the direction of technology innovations. It has been found that the femtocells and mobile nodes in cellular network communications can benefit from the introduction of \acp{UAV}. This could be increasingly useful in the mmWave and 5G perspectives. Further research efforts should be spent in this direction, even if some works have already addressed this issue, since this is a promising research field to improve communication and data exchange in different hybrid scenarios.

The existing evaluations about interoperability and seamless communications can be extended in several directions.
Given the heterogeneity of the available technologies, a key role can be played by middleware solutions enabling the interactions among the drones forming swarms as well as between the drones and the ground infrastructure.

Interface software and middleware solutions can be considered as key elements in communications but also in the data processing phase. This consideration is not only applicable to the \acp{UAV} equipment but also at the ground network level.

As for communications among drones, the main trends are related to the extension of the covered area and the employability of communication protocols to guarantee a target \ac{QoE} in both \ac{A2A} and \ac{A2G}. In the 5G perspective, it could be useful to standardize communications and creating homogeneous frameworks and platforms that provide real integration among heterogeneous technologies, rather than pushing on performance (e.g., increasing the data rate or decreasing latencies). This process is often referred to as \textit{Softwarization}.
It is worth noting that a similar phenomenon is taking place in the \ac{IoT} world., where a number of examples and dedicated studies are specifically focused at integrating the existing \ac{IoT} technologies rather than developing new ones \cite{GBF+16, BDP+16, ZPS+18, MMN+17}. Specific attention is devoted to the security aspects of such interactions \cite{SKP+18}, thus proposing innovative solutions based on Blockchain and smart contracts \cite{RMC+18}.

Another example can be found in the application of \acp{VLC} and \ac{ICN} technologies to drones.
Some works have already contributed on the \ac{VLC} topic \cite{YCL14,CD17,RRL12,SKU16,MBM14,WGP14,LTK+12,WWY14,YTO+14}, especially for what concerns the analysis of the IEEE standards \cite{YCL14}, modulation schema and light patterns at physical layer \cite{RRL12}, MAC layer analysis and performance of network topologies \cite{SKU16,MBM14}, simulation software \cite{MBM14,WGP14}, applications of the \ac{VLC} system architecture \cite{LTK+12,YTO+14} with its strengths and weaknesses  \cite{WWY14}, and related performance evaluation \cite{CD17}. It would be very interesting, as a future research direction, to investigate the possibilities of application of this novel technology to the \ac{IoD} field.

Another research challenge in drone communication concerns security and privacy in data exchange. Strictly related to privacy is the legislation issue. Legislative interventions could also be of importance on the theme of privacy, even if some problems have still to be solved \cite{DWZ+18}. In particular, one of the concerns is related to the idea that drones moving all along urban and suburban areas could impair privacy of the people. To the best of the authors knowledge, very few works analyze these aspects: the work \cite{WSB15} treats these themes from a technological point of view, for example securing transmission and reception activities. The contribution \cite{LHK+18} specifically addresses privacy issues of the \ac{IoD} in both civilian and military architectures and a certain number of security and privacy requirements. The work \cite{PBC14} raises a flag from the privacy and resource accessibility points of view, which should absolutely not be set free in communication networks of any kind. Nevertheless, research efforts could be made in this direction to further analyze and improve these aspects. 

Another interesting research line that definitely deserves attention is the application of \ac{ICN} in the context of the \ac{IoD} \cite{BLP+18}.
In particular, what clearly emerges from the study of the related state-of-the-art, is that the application of the \ac{ICN} in the context of \acp{ITS} seems not to be already as mature as it could \cite{STG16, CM16}.
As a matter of fact, the authors believe that this may represent a limiting factor since the \ac{ICN} architecture proposes one of the best solutions to support communications over users, especially in mobile-by-design scenarios \cite{Kerrche2020,SA18A}.
Among the main reasons that make this of relevance, there is the increasingly emerging limitation of the host-centric nature of the Internet, as known today.
Indeed, there is a continuous request for seamless mobility, coming from users of different nature, and pushing to the limit the Internet capabilities.
The proper support to intrinsic mobile scenarios becomes necessary in those cases in which the handover is frequently verified. The latter is, in fact, an extremely well-known problem in the telecommunications world as, in a mobile scenario, the user remains connected to the network, and does not experience any discontinuity of service, if, and only if, the coverage is acceptable.
Since the global connectivity cannot be granted by using a single access point (i.e., a single cell in the case of cellular networks), the problem of the handover arises when the user moves from one access point to another. In the case of cellular networks, this happens when the user moves from one cell to one of the neighboring ones.
The intrinsic mobility that characterizes \acp{ITS} systems, both from the points of view of users and drones producing data, places serious constraints on sustainability.
It is worth noting that routing problems also arise in these cases, because of the need to realize in real-time which access point is the \ac{UAV} connected to, and both in \ac{DL} and \ac{UL}. If the routes are not known, the \ac{UAV} will experience a loss of connectivity and information exchange.
The \ac{ICN} communication paradigm leveraging the Publish-Subscribe communication scheme represents a good candidate for granting \ac{QoS} design criteria, for instance communication latencies, \ac{PLR}, resilience, and throughput. The joint analysis of even some of these aspects, combined together in \ac{ITS} applications, could be an interesting challenge for the future research.

Some other considerations are related to technology and to the massive production and widespread diffusion of autonomous vehicles, even more so in industrial applications. It is well known that there is a close relationship between costs and the development of a technology \cite{LALL1992165}. In this context, advanced industrial countries select, and apply without costs, all the innovations that are more immediately useful. As the general level of capital accumulation rises, more capital-intensive technologies become economical.
Since industrialization is driven by technology applicability, and considerably boosted by rapid prototyping, the need for a drone to carry out part of industrial process monitoring or supply chain support/optimization depends on its cost and its accessibility.
The consideration can be completed by reasoning on the legal aspects of the question. Since there is not a unified legislation on the usage of unmanned vehicles, the seamless employability is still far from now. In a globalized economy context, this means that a firm or an industry may find economical and legal barriers to their welcoming attitude towards drones. In all the analyzed works, these aspects have been neglected, but they surely represent a value added in future research on the \ac{IoD} theme.
